Toward a Blockchain-based Platform to Manage Cybersecurity Certification of IoT devices

The goal of this paper is to propose a blockchain-based platform to enhance transparency and traceability of cybersecurity certification information motivated by the recently adopted EU Cybersecurity Act. The proposed platform is generic and intended to support the trusted exchange of cybersecurity certification information for any electronic product, service, or process. However, for the purposes of this paper, we focus on the case study of the cybersecurity certification of IoT devices, which are explicitly referenced in the recently adopted Cybersecurity Act as one of the main domains where it is highlighted the need for an increased level of trust.

==> iot.tex <==
\section{Scenario description}
\label{sec:iot}



==> related-work.tex <==
\section{Related Work}
\label{sec:related-work}


